Are Language Models Puzzle Prodigies? Algorithmic Puzzles Unveil Serious Challenges in Multimodal Reasoning

This paper introduces the novel task of multimodal puzzle solving, framed within the context of visual question-answering. We present a new dataset, AlgoPuzzleVQA designed to challenge and evaluate the capabilities of multimodal language models in solving algorithmic puzzles that necessitate both visual understanding, language understanding, and complex algorithmic reasoning. We create the puzzles to encompass a diverse array of mathematical and algorithmic topics such as boolean logic, combinatorics, graph theory, optimization, search, etc., aiming to evaluate the gap between visual data interpretation and algorithmic problem-solving skills. The dataset is generated automatically from code authored by humans. All our puzzles have exact solutions that can be found from the algorithm without tedious human calculations. It ensures that our dataset can be scaled up arbitrarily in terms of reasoning complexity and dataset size. Our investigation reveals that large language models (LLMs) such as GPT4V and Gemini exhibit limited performance in puzzle-solving tasks. We find that their performance is near random in a multi-choice question-answering setup for a significant number of puzzles. The findings emphasize the challenges of integrating visual, language, and algorithmic knowledge for solving complex reasoning problems.

==> category_results.tex <==
\begin{table*}[ht]
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cccc}
\toprule[1pt]
\multirow{2}{*}{\textbf{Ontology}} & \multicolumn{2}{c|}{\textbf{CoT}} & \multicolumn{2}{c|}{\textbf{Elaborate CoT}} & \multirow{2}{*}{\textbf{InstructBLIP}} & \multirow{2}{*}{\textbf{Qwen-VL}} & \multirow{2}{*}{\textbf{LLaVa}}\\
& \textbf{GPT-4V} & \textbf{Gemini Pro} & \textbf{GPT-4V} & \textbf{Gemini Pro} \\
\midrule 
\textbf{Visual Features} &  &  &  &  &  & &  \\
\qquad Colour &  &  &  &  &  & &  \\
\qquad Position &  &  &  &  &  & &  \\
\qquad Shape/Size &  &  &  &  &  & &  \\
\qquad Text &  &  &  &  &  & &  \\
\midrule 
\textbf{Algorithmic Features} &  &  &  &  &  & &  \\
\qquad Arithmetic &  &  &  &  &  & &  \\
\qquad Boolean Logic &  &  &  &  &  & &  \\
\qquad Combinatorics &  &  &  &  &  & &  \\
\qquad Graphs &  &  &  &  &  & &  \\
\qquad Optimization &  &  &  &  &  & &  \\
\qquad Search &  &  &  &  &  & &  \\
\qquad Sets &  &  &  &  &  & &  \\
\bottomrule
\end{tabular}
}
\caption{Results across all the ontological categories for the various multimodal language models.}
\label{tab:results_category}
\end{table*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> puzzle_details.tex <==
\subsection{Board Tiling}\label{sec:board_tile}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{images/board_tile_0003.pdf}
  \caption{\small{\texttt{\textbf{Question:} The checkerboard shown in the image was originally of 6 * 9 in dimension having a total of 54 squares. It uses two colours of squares, one light yellow and one dark yellow, in a chequered pattern. Two of the squares have been removed from the board in the position of the white coloured cells, as shown in the image. You have 26 dominoes of size 2 * 1. You can use them as is or you can rotate them to use as a 1 * 2 domino. Is it possible to place all the 26 dominoes in the checkerboard to exactly cover all the remaining 52 squares? Answer Yes or No. \textbf{Gold Answer:} Yes}}}
  \label{fig:board_tile}
\end{figure}

The puzzle is inspired by the Mutilated chessboard problem, originally posed by Max Black~\citep{black1948critical}. It is a domino tiling puzzle which asks: \textit{Suppose a standard $8 * 8$ chessboard has two diagonally opposite corners removed, leaving 62 squares. Is it possible to place 31 dominoes of size $2 * 1$ to cover all of these squares?} The diagonally opposite corners in a standard $8 * 8$ chessboard are always of the same colour. Hence, the mutilated chessboard with $62$ squares has $30$ squares of one colour and $32$ squares of the other colour. Now, the checkered pattern of the chessboard ensures that each $2 * 1$ domino must cover $1$ dark-coloured square and $1$ light-coloured square. It is thus impossible to place the dominoes to cover all the squares since the mutilated chessboard has an unequal number of dark and light-coloured squares.

An extension of the puzzle asks whether an $8 * 8$ chessboard is always tileable if \textit{any} two squares of opposite colours are removed. This was unanswered for several years until a proof by Gomory appeared in \emph{Mathematical Gems I} by \citet{honsberger1973mathematical}. The proof has later been extended to any sized checkboard ~\citep{mendelsohn2004tiling} with the following key results: 

\begin{enumerate}[leftmargin=9mm]
    \item A checkerboard originally had an even number of squares: $2 * m + 2$. If two squares are removed from the board then the mutilated board is tileable with $m$ dominoes of size $2 * 1$ iff the removed squares are of the opposite colour. Otherwise, it is not tileable.
    \item A checkerboard originally had an odd number of squares: $2 * m + 1$. If one square is removed from the board then the mutilated board is tileable with $m$ dominoes of size $2 * 1$ iff the mutilated board has an equal number of dark and light squares. Otherwise, it is not tileable.
\end{enumerate}

We use this result to construct our puzzles. We choose the number of rows and columns in our checkerboard randomly between $4$ to $9$. We randomly remove $1$ or $2$ squares if the board has an odd or even number of squares, respectively. We question whether the resulting board is tileable with $m$ dominoes of size $2 * 1$. We determine the yes or no answer based on the colour of the removed square(s). We show an example of the puzzle in \Cref{tab:examples1}.

\subsection{Box Pushing}\label{sec:box_push}

\subsection{Calendar}\label{sec:calendar}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.55\textwidth]{images/calendar_0001.pdf}
  \caption{\small{\texttt{\textbf{Question:} The image shows the calendar of a month of a particular non-leap year. Which day of the week was on March 1 of that year? \textbf{Gold Answer:} Friday}}}
  \label{fig:calendar}
\end{figure}

We design this puzzle to evaluate the visual-temporal reasoning abilities of foundation models. We provide the calendar snapshot of a particular month as the visual context. We then ask what day of the week was a particular date in either the previous, same or the next year. We also provide information about whether the years of consideration were leap years or not to make sure that the answer is exact. We use the python \textit{calendar} module to construct the instances of the puzzle. We show an example of the puzzle in \Cref{tab:examples1}.

\subsection{Chain Link}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.75\textwidth]{images/chain_link_0000.pdf}
  \caption{\small{\texttt{\textbf{Question:} Alice has 12 segments of chains of different lengths as shown in the image. The total length of all the segments combined is 32 pieces. She has a saw machine with which a closed piece can be cut opened. She also has a welding machine with which an open piece can be closed. Each cut takes 5 minutes and each welding takes 2 minutes. Initially, she has 3 segments each with 1 open piece as shown in the image. All the other pieces are closed. She now wants to make the longest possible necklace using all the available 32 pieces. Each piece in the necklace would be connected to exactly two other pieces. This would require cutting open some pieces and then joining all the resulting segments together. What is the minimum time in which she can create the necklace? \textbf{Gold Answer:} 34}}}
  \label{fig:chain_link}
\end{figure}

This puzzle is a modified version of a similar problem which appeared in the \emph{The Moscow Puzzles}~\citep{kordemsky1992moscow}. The puzzle states that you are given chain segments of different lengths. Some of the segments of unit piece length are initially open, whereas the others are closed. Closed pieces can be cut open and open pieces can be welded together in a certain amount of time. You need to create the longest possible circular necklace using all the pieces where each piece is connected to exactly two other pieces. The objective is to create the necklace using the least possible cuts and joins, resulting in the least possible time required. We show an example of the puzzle in \Cref{tab:examples1}.

The puzzle can be solved optimally using the following strategy:

\begin{enumerate}[leftmargin=6mm]
    \item Check if the number of open links is equal to or greater than the number of closed segments. We can weld together all the pieces into the longest possible necklace when this is satisfied. Initially, in our example, the number of open links is $3$ and the number of closed segments is $9$. The condition is not satisfied and hence we move to the next step.
    \item  Cut open units from the segments of the least length until the first condition is satisfied. In our example, if you cut open the two segments of length $1$ and both the units in the segment with length $2$ then you have $4$ additional open links. Now the total number of open links is $7$ and the number of closed segments is $6$. The first condition is now satisfied.
    \item Calculate the time required considering the total number of cuts and welds required. We performed $4$ cut operations and then we will need $7$ welding operations to close all the open links. The total time required is $4 * 5 + 7 * 2 = 34$ minutes. This is the minimum possible time required to create the necklace. 
\end{enumerate}

\subsection{Clock}
\begin{figure}[h]
  \centering
  \includegraphics[width=0.4\textwidth]{images/clock_0000.pdf}
  \caption{\small{\texttt{\textbf{Question:} Alexis came to an event 3 minutes ago. The current time is shown on the clock. The clock is a standard analog clock without the seconds hand. What was the time when Alexis came to the event? \textbf{Gold Answer:} 9:19}}}
  \label{fig:clock}
\end{figure}

We design another instance of a visual-temporal reasoning puzzle using clock times. We consider an analog clock with the hours and minutes hand and show a randomly chosen time as the visual context. The time shown in the clock is considered as the current time. We also describe an event which happened $h$ hours and $m$ minutes ago or is going to happen $h$ hours and $m$ minutes later. We then ask when did the event happen or when is it going to happen as the question. We determine the answer using modular arithmetic. We show an example of the puzzle in \Cref{fig:clock}.

\subsection{Colour Hue}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.6\textwidth]{images/colour_hue_0022.pdf}
  \caption{\small{\texttt{\textbf{Question:} A 5 * 4 board consists of 20 different coloured tiles. A random state of the board is shown in (A). The ideal state of the board is shown in (B). A swap consists of selecting any two tiles in the board and switching their positions. What is the minimum number of swaps required to restore the ideal state of the board from (A)? \textbf{Gold Answer:} 4}}}
  \label{fig:colour_hue}
\end{figure}

The puzzle is inspired by the game \emph{I Love Hue}\footnote{\url{https://i-love-hue.com/}}. A board contains of $m * n$ coloured tiles arranged in a rectangular grid. The board has an ideal state where the colours are arranged in a way such that each row and column shows a monotonic change in the colour shade. To create this colour arrangement, we fix the RGB colour codes of the four corner tiles and perform linear interpolation between them to determine the colour codes of the intermediate tiles. We then randomly shuffle some of the tiles to create a non-ideal arrangement of the board. We ask how many minimum tile swaps are required to reach the ideal state from the non-ideal state. 

The answer can be determined using the selection sort algorithm, which minimizes the number of swaps required to sort an unsorted array. We consider the flattened version of the ideal state of the board to be the sorted state. The flattened version of the non-ideal state of the board is considered as the unsorted state. We then determine the answer using selection sort. We show an example of the puzzle in \Cref{fig:colour_hue}.



% \subsection{Geomagic Square}

\subsection{Map Colouring}
\begin{figure}[h]
  \centering
  \includegraphics[width=0.45\textwidth]{images/map_0029.pdf}
  \caption{\small{\texttt{\textbf{Question:} You are given an incomplete map of a country having 15 different regions. The objective is to colour the regions of the map using only the four available colours: red, green, blue and yellow, such that no two adjacent regions have the same colour. Adjacent regions are defined as two regions that share a common boundary of non-zero length. The regions indicated by numbers 1 to 10 have already been coloured, as shown in the image. The regions indicated by numbers 11 to 15 are shown in white as they are yet to be coloured. You need to assign colours to these regions in a way such that it doesn't violate the objective. Each unique colour combination of the regions would result in a unique complete map. How many unique complete maps can be created by colouring all the white regions starting from the given incomplete map? \textbf{Gold Answer:} 8}}}
  \label{fig:map}
\end{figure}

The four colour theorem is a famous result in mathematics which states that four colors are sufficient to color the regions of any planar map such that no two adjacent regions have the same color. The conjecture was first proposed in the 1850s but a formal proof \citep{appel1977solution} was first developed almost 120 years later.

We show an example of the puzzle in \Cref{fig:map}. To construct this puzzle, we first create a Voronoi diagram from a finite set of points \citep{Voronoi1908}. We then use the polygon clipping algorithm \citep{sutherland1974reentrant} to clip the Voronoi diagram between the finite regions of $(x, y)$, where $0 \leq x \leq 1$ and $0 \leq y \leq 1$. This region constitutes our input map. We represent the map as a graph with regions as nodes and their adjacent regions as the adjacency list. We use graph colouring strategy based on Algorithm X \citep{knuth2000dancing} with four colours to find the exhaustive solutions for colouring the map. We fix the colours of some of the regions of the map and mask the colours of the rest. We can then find out the number of ways the masked regions can be coloured from the exhaustive list of solutions. We construct the puzzles in our dataset such that the number of masked regions is between $2$ and $6$ and the number of ways of colouring them is between $1$ and $8$. 

\subsection{Maze Solving}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{images/maze_0001.pdf}
  \caption{\small{\texttt{\textbf{Question:} This is maze having 13 * 13 cells. The empty cells are coloured white and the obstacle cells are coloured black. From an empty cell, you can only move up, down, left, or right to another adjacent empty cell. You cannot move diagonally between two empty cells and cannot step into a cell with an obstacle. The entry cell of the maze is shown with the green arrow. The exit cell of the maze is shown with the blue arrow. Suppose you have found the most optimal path in the maze between the entrance and exit, where you need to go through the least number of empty cells and you need to make the least number of left and right turns. What is the combined number of left and right turns do you need to make in this optimal path? \textbf{Gold Answer:} 12}}}
  \label{fig:maze}
\end{figure}

This puzzle is a typical maze path-finding problem. We start from a square/rectangular grid consisting of all black cells (walls). We define the first cell of the second row as the entrance to the maze. We then perform a directionally randomized depth-first search (DFS) with backtracking from the entrance cell to create the white cells (paths) through the maze. We also make sure that at any point of the maze, either the maximum length or the maximum width of the path is $1$ cell. This method ensures that there are no grids of white cells in the maze with both length and width greater than $2$. We finally assign the last column of the second last row or the last row of the second last column as the exit cell.

After constructing the maze, we use breadth-first search (BFS) between the entrance cell and the exit cell to find the shortest / optimal path. We then randomly select one question for this instance among the following choices:

\begin{itemize}[leftmargin=6mm,itemsep=-0.1mm]
    \item What is the total number of left turns do you need to make in this optimal path?
    \item What is the total number of right turns do you need to make in this optimal path?
    \item What is the combined number of left and right turns do you need to make in this optimal path?
    \item How many cells do you need to visit in this optimal path including the entrance and exit cells?
\end{itemize}

We find out the answer to the question from the optimal path obtained from BFS. We show an example of the puzzle in \Cref{fig:maze}.

\subsection{N-Queens}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.45\textwidth]{images/n_queens_0000.pdf}
  \caption{\small{\texttt{\textbf{Question:} You are given an 8 * 8 chessboard. The Manhattan distance between two squares in a chessboard is equal to the minimal number of orthogonal King moves between these squares on the otherwise empty board. The objective is to place 8 chess queens on this board so that no two queens threaten each other; i.e. no two queens share the same row, column, or diagonal. 6 queens have already been placed in some of the squares of the board, as shown in the image. Suppose you pick two squares to place the two remaining queen pieces in a way that fulfills the objective. What is the Manhattan distance between these two squares? \textbf{Gold Answer:} 5}}}
  \label{fig:n_queens}
\end{figure}

The N-Queens problem is a famous chess problem often used as an example in various computer programming techniques. The objective of this problem is to place $N$ chess queens on an $N * N$ chessboard so that no two queens threaten each other. In other words, no two queens should share the same row, column, or diagonal. We consider $N = 8, 9,$ and $10$ for which there are $92, 352,$ and $724$ solutions, respectively. 

We consider these solutions to create the instances of our puzzle. For a solution, we show the exact position of randomly chosen $N-2$ queens in the image. We ask what should be the Manhattan distance (in terms of the unit squares of the board) between the remaining $2$ queens when they are placed correctly to satisfy the objective.
The other $2$ queens can be arranged in only a single way for most cases, for which we can easily compute the Manhattan distance. In some minimal number of cases, the other $2$ queens can be placed in two different ways to satisfy the non-threatening condition in all rows, columns, and diagonals. However, in both of these ways, the Manhattan distance between the last $2$ queens is equal. So, we can have an exact answer to the question even though the arrangement could be distinct. We show an example of the puzzle in \Cref{fig:n_queens}.

\subsection{Number Path}

\subsection{Number Slide}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.4\textwidth]{images/number_slide_0009.pdf}
  \caption{\small{\texttt{\textbf{Question:} The board shown in the image is a sliding puzzle of 4 * 4 tile dimensions. It has 15 numbered tiles and one unoccupied (open) position. Tiles in the same row or column of the open position can be moved by sliding them horizontally or vertically, respectively. All tiles always stay and move inside the red boundary wall, as shown in the image. A move is defined as moving the open position by one tile unit in any available direction. You start from the board position shown in the image and perform exactly 1 move. What is the minimum sum that you can achieve across the top most row in the final board position? \textbf{Gold Answer:} 22}}}
  \label{fig:number_slide}
\end{figure}

This puzzle is inspired by the mathematical toy known as the $15$ Puzzle\footnote{\url{https://en.wikipedia.org/wiki/15_Puzzle}}. It is a sliding puzzle board of grid size $4 * 4$. It has $15$ square tiles numbered 1 to 15 in the frame, with one unoccupied position. Tiles can be moved by sliding them horizontally or vertically through the open position. A typical goal in the puzzle is to arrange the tiles in numerical order from left to right and top to bottom.

We use grid sizes of $3 * 3, 4 * 4,$ or $5 * 5$ and create a random arrangement of the tiles on the board and provide it as the visual context. We then create the question in one of the following styles:

\begin{itemize}[leftmargin=8mm]
    \item How many unique board positions can be reached after performing exactly $n$ moves?
    \item What is the maximum / minimum sum that can be achieved in a  particular row / column after performing exactly $n$ moves? 
    \item You perform $n$ moves where the open position is seen to be moved in the following way: \textit{up, left, \dots}. What is the maximum / minimum / sum of numbers in the row / column that now has the open position? 
\end{itemize}

We compute the answer using breadth-first search in all the cases. We show an example of the puzzle in \Cref{fig:number_slide}.

\subsection{Rotting Fruit}

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.4\textwidth]{images/rotting_kiwi_0000.pdf}
  \caption{\small{\texttt{\textbf{Question:} You are given a 3 x 3 grid in which each cell can contain either no kiwi, one fresh kiwi, or one rotten kiwi. Every minute, any fresh kiwi that is 4-directionally adjacent to a rotten kiwi also becomes rotten. What is the minimum number of minutes that must elapse until no cell has a fresh kiwi? \textbf{Gold Answer:} 3}}}
  \label{fig:rotting_kiwi}
\end{figure}

\subsection{Rubik's Cube}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{images/rubiks_cube_0041.pdf}
  \caption{\small{\texttt{\textbf{Question:} A 3 * 3 Rubik's Cube has six different coloured panels: red, green, blue, yellow, orange, and grey. The initial state of the cube in terms of the different colour positions in its six faces is shown in the image. To represent the movements of the cube we use six letters: U for Up, D for Down, L for Left, R for Right, F for Front, B for Back. These letters are used in sequence where you need to perform each letter in the sequence from left to right. Each letter tells you to move that face clockwise by 90 degrees. A number 'n' immediately after a letter denotes that you need to move that face clockwise by 90 * n degrees. For example, `U R3' would mean rotating the up face 90 degrees clockwise and then rotating the right face 270 degrees clockwise. You perform the move sequence `D2 B' starting from the state shown in the image. What would be the number of small 1 * 1 red squares in the down face after completing the move sequence? \textbf{Gold Answer:} 22}}}
  \label{fig:rubiks_cube}
\end{figure}

Rubik's Cube is a famous mathematical combination toy invented by Ernő Rubik in 1974. We consider an initial state of the cube and show it as the visual context. The movements of the cube are generally denoted using the alphabets \textsc{BDFLRU} denoting clockwise movements of the back, down, front, left, right, and up faces, respectively. We first provide information about these notations in the textual context. We then ask what is the number of small squares of any one of the six colours in any one of the six faces after completing a move sequence. The colour and the face in the question are chosen randomly for each instance. We show an example of the puzzle in \Cref{fig:rubiks_cube}.

\subsection{Think A Dot}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{images/think_dot_0050.pdf}
  \caption{\small{\texttt{\textbf{Question:} The toy shown in the figure has eight coloured disks on its front, and three holes on its top - left, right, and center - through which a ball bearing could be dropped. Each disk would display either a yellow or blue face. When a ball passes through a disc it tips the disk mechanism which flips the face color. The tipping of the disc mechanism determines whether the ball would be deflected to the left or to the right. The vertical walls between the discs would then determine the path of motion of the ball. A dropped ball always passes through exactly one disc in each of the top and the bottom row. Depending on the configuration of the top three discs it may or may not pass through the middle row. Finally, when the ball falls to the bottom it would exit either to a hole on the left or the right of the device. Four balls are dropped in sequence through the following holes: left, left, right, right. Consider the toy configuration after all the balls have been dropped and they have exited from the bottom. How many yellow faces can be seen in total in all the rows now? \textbf{Gold Answer:} 6}}}
  \label{fig:think_dot}
\end{figure}

Think-a-Dot is a mathematical toy invented by Joseph Weisbecker\footnote{\url{https://en.wikipedia.org/wiki/Think-a-Dot}}. It has three holes on its top through which a ball bearing could be dropped. It also has eight coloured disks on its front each displaying a blue or yellow face, depending on the direction towards which the mechanism behind it was tipped. When a ball is dropped through the toy, it would flip the disk mechanisms that it passed, and they in turn would determine whether the ball would be deflected to the left or the right. 

We show an example of the puzzle in \Cref{fig:think_dot}. We start with an initial configuration of the toy with a specific combination of the disk colours. We choose between $1$ to $4$ balls and choose a sequence of dropping them between the left, center and right holes. We then ask how many blue / yellow disk faces can be seen in the top row / middle row / bottom rows / all rows after dropping all the balls in that sequence. 

We write an algorithm to determine the answer from the initial configuration and the sequence of drops. The algorithm considers the current state of each row and determines which way the ball would be deflected constrained upon the flipped disk and the position of the walls. This information is then used to determine the state of the next row. 
 
\subsection{Tower of Hanoi}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.6\textwidth]{images/tower_of_hanoi_0004.pdf}
  \caption{\small{\texttt{\textbf{Question:} You are playing a Tower of Hanoi game with 3 rods and 5 disks of various diameters, which can slide onto any rod. You are given the starting and ending configuration of the game as shown in the top and the bottom of the image, respectively. The game has the following rules: i) Only one disk may be moved at a time; ii) Each move consists of taking the upper disk from one of the stacks and placing it on top of another stack or on an empty rod; and iii) No disk can be placed on top of a disk that is smaller than it. What is the minimum number of moves required to go from the starting to the ending configuration? \textbf{Gold Answer:} 2}}}
  \label{fig:tower_of_hanoi}
\end{figure}

The Tower of Hanoi is a well-known mathematical game often used in teaching the fundamentals of computer programming. The game consists of $3$ rods and $n$ disks of various diameters, that can slide into any rod. In the original version of the puzzle, we start with all the disks stacked on one rod in order of decreasing size. The goal is to move the full stack of disks to another rod
% Moving the discs between the rods is constrained by some rules as defined in our example in \Cref{fig:tower_of_hanoi}.
constrained by the following rules: (i) We can only move one disc at a time, (ii) Each move consists of taking the upper disk from one of the stacks and placing it on top of another stack or on an empty rod, (iii) No disk can be placed on top of a disk that is smaller than it. With no other constraints, the puzzle can be solved in a minimum of $2^n - 1$ moves. 

We consider the number of discs to be between $3$ and $6$ for our dataset. We generate the optimal solutions considering the original problem definition. We then select two random configurations of the game from the optimal solution, which are at most $k = 6$ moves away from each other. We consider them to be the starting and the ending configuration. As the original solution is optimal, the sequence of moves required to reach the ending configuration from the starting configuration is also optimal. We ask what is the minimum number of moves required to reach the ending configuration from the starting configuration. We mark the answer to be $k$. We show an example of the puzzle in \Cref{fig:tower_of_hanoi}.

\subsection{Water Jugs}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{images/water_jugs_0000.pdf}
  \caption{\small{\texttt{\textbf{Question:} You are given 3 jugs of capacities 6, 5, 1 litres. Initially, the amount of water that is contained in each jar is shown in the image. A single step of water pouring from one jug to another is constrained by the following rules: i) take a non-empty jug and pour water from it to another non-full jug until the first one becomes empty or the second one becomes full, and ii) no water can be spilt while pouring. The objective is to reach the amounts of 4, 3, 0 litres of water in the jugs from left to right, respectively. What is the minimum number of water pouring steps required to achieve the objective? \textbf{Gold Answer:} 1}}}
  \label{fig:water_jugs}
\end{figure}

This puzzle belongs to a class of measuring puzzles involving a finite collection of water jugs with integer capacities. We provide the initial amount of water present in each jug as the visual context. We then ask how many steps of water pouring are required to reach a goal state defined in terms of specific quantities of water present in each jug. The water pouring steps are constrained by a couple of rules: i) water can be poured from a non-empty jug to another non-full jug until the first one becomes empty or the second one becomes full, and ii) no water can be split during the pouring process. 

We consider the number of jugs to be between $3$ and $5$, with each initially having an amount between $1$ and $14$ litres of water. We create a pool of random goal states having the same quantity of total water with each jug having water that is less or equal to its respective capacity. We compute if the goal state is reachable using breadth-first search and only consider goal states which are at most 5 moves away from the initial state. We use these instances for our dataset. We show an example of the puzzle in \Cref{fig:water_jugs}.

\subsection{Wheel of Fortune}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{images/wheel_of_fortune_0010.pdf}
  \caption{\small{\texttt{\textbf{Question:} A fortune wheel has 6 segments of different colour. The initial position of the wheel is shown in the figure. Each segment is associated with a prize as shown in the embedded text within the segment. The axis of rotation of the wheel passes through its center and is perpendicular to the surface of the wheel. You spin the wheel counterclockwise and it rotates 465 degrees before stopping. You are going to win the prize for the segment that now falls in front of the brown arrow. What is your prize? \textbf{Gold Answer:} Jewelry}}}
  \label{fig:wheel_of_fortune}
\end{figure}

We design this spinning wheel puzzle to assess the spatial reasoning ability of foundation models. We sketch a wheel with $6,  8$ or $10$ segments with different colours and associate each of them with a prize. The angular span of the segments is chosen to be either uniform or random. We show the initial position of the wheel and the position of a fixed arrow as the visual context. We then ask what the prize would be (from the segment in front of the arrow) after the wheel has been rotated by a certain amount of degrees or full rotations in either clockwise or anti-clockwise direction. We determine the answer using simple rotational mechanics. We show an example of the puzzle in \Cref{fig:wheel_of_fortune}.

\subsection{Wood Slide}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\textwidth]{images/wood_slide_0001.pdf}
  \caption{\small{\texttt{\textbf{Question:} Consider a sliding block puzzle of grid size 5 * 4 units. It has 9 wooden blocks of varying sizes: one 2 * 2, four 1 * 2, two 2 * 1, and two 1 * 1. The gird also has two empty 1 * 1 spaces. The blocks cannot be removed from the grid, and may only be slid horizontally and vertically within its boundary. A move is defined as selecting a block that is slideable, and moving it by 1 unit either horizontally or vertically, whichever is possible. The image shows the starting and ending configurations of the puzzle grid. The wooden blocks are shown in various shades of brown and the empty spaces are shown in white. What is the minimum number of moves required to reach the ending configuration from the starting configuration? \textbf{Gold Answer:} 3}}}
  \label{fig:wood_slide}
\end{figure}

This puzzle is inspired by the Klotski\footnote{\url{https://en.wikipedia.org/wiki/Klotski}} sliding puzzle. We consider a puzzle grid of size 5 * 4 units that has 9 wooden blocks of various sizes: one 2 * 2, four 1 * 2, two 2 * 1, and two 1 * 1. The other two spaces are empty. There is a version of the Klotski puzzle known as the Pennant Puzzle where we start with the largest 2 * 2 block residing at the top left. The objective is to bring this piece to the bottom left by sliding the available pieces. The shortest solution of this puzzle consists of 83 moves. We first use breadth-first search to find this optimal solution. For each instance in our dataset, we choose two board positions encountered in this solution such that they are at most 5 moves away from each other. We consider these positions as the starting and ending configuration of the board. We then create the question that asks the minimum number of moves required to reach the ending configuration from the starting configuration. We show an example of the puzzle in \Cref{fig:wood_slide}.

==> puzzle_table1.tex <==
\begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{m{7cm} m{8cm}}
\toprule
\multicolumn{1}{c}{\textbf{Image}} & \multicolumn{1}{c}{\textbf{Question and Answer}} \\
\midrule

\includegraphics[width=7cm, height=4.5cm]{images/board_tile_0003.pdf} & 
\vspace{-2cm}
\parbox{8cm}{\small{\texttt{\textbf{Question:} The checkerboard shown in the image was originally of 6 * 9 in dimension having a total of 54 squares. It uses two colours of squares, one light yellow and one dark yellow, in a chequered pattern. Two of the squares have been removed from the board in the position of the white coloured cells, as shown in the image. You have 26 dominoes of size 2 * 1. You can use them as is or you can rotate them to use as a 1 * 2 domino. Is it possible to place all the 26 dominoes in the checkerboard to exactly cover all the remaining 52 squares? Answer Yes or No. \\
\textbf{Gold Answer:} Yes}}} \\

\midrule

\midrule

\includegraphics[width=7cm,height=5cm]{images/calendar_0001.pdf} \vspace{-1cm} &
\parbox{8cm}{\small{\texttt{\textbf{Question:} The image shows the calendar of a month of a particular non-leap year. Which day of the week was on March 1 of that year? \\
\textbf{Gold Answer:} Friday}}} \\
  
\midrule

\vspace{0.25cm}
\includegraphics[width=7cm, height=5.5cm]{images/chain_link_0000.pdf} &
\vspace{-3cm}
\parbox{8cm}{\small{\texttt{\textbf{Question:} Alice has 12 segments of chains of different lengths as shown in the image. The total length of all the segments combined is 32 pieces. She has a saw machine with which a closed piece can be cut opened. She also has a welding machine with which an open piece can be closed. Each cut takes 5 minutes and each welding takes 2 minutes. Initially, she has 3 segments each with 1 open piece as shown in the image. All the other pieces are closed. She now wants to make the longest possible necklace using all the available 32 pieces. Each piece in the necklace would be connected to exactly two other pieces. This would require cutting open some pieces and then joining all the resulting segments together. What is the minimum time in which she can create the necklace? \\
\textbf{Gold Answer:} 34}}} \\

\bottomrule
\end{tabular}
}
\caption{Examples of Board Tiling, Box Push, Calendar and Chain Link puzzles.}
\label{tab:examples1}
\end{table}
